Towards Dynamic and Safe Configuration Tuning for Cloud Databases

Configuration knobs of database systems are essential to achieve high throughput and low latency. Recently, automatic tuning systems using machine learning methods (ML) have shown to find better configurations compared to experienced database administrators (DBAs). However, there are still gaps to apply the existing systems in production environments, especially in the cloud. First, they conduct tuning for a given workload within a limited time window and ignore the dynamicity of workloads and data. Second, they rely on a copied instance and do not consider the availability of the database when sampling configurations, making the tuning expensive, delayed, and unsafe. To fill these gaps, we propose OnlineTune, which tunes the online databases safely in changing cloud environments. To accommodate the dynamicity, OnlineTune embeds the environmental factors as context feature and adopts contextual Bayesian Optimization with context space partition to optimize the database adaptively and scalably. To pursue safety during tuning, we leverage the black-box and the white-box knowledge to evaluate the safety of configurations and propose a safe exploration strategy via subspace adaptation.%, greatly decreasing the risks of applying bad configurations. We conduct evaluations on dynamic workloads from benchmarks and real-world workloads. Compared with the state-of-the-art methods, OnlineTune achieves 14.4%~165.3% improvement on cumulative performance while reducing 91.0%~99.5% unsafe configuration recommendations.

==> exp_old.tex <==
\section{EVALUATION}
%In this section, we evaluate the performance of \sys. 

\noindent\textbf{Experiment Outline}:
 We first compare  \sys with the-state-of-art database knobs tuning methods on \textit{static workload} setting, an evaluation setting existing auto-tuner used.
 Then we conduct end-to-end evaluations in three setting: (1) \textit{dynamic workload}, where queries composition is constantly changing, (2) \textit{transactional-analytical}, simulating a daily transactional-analytical workload cycle by alternating the execution of OLTP and OLAP workload, (3) \textit{real-workload workload}. Then, we conduct ablation studies to evaluate the effectiveness of \sys's design, including context space design and safe optimization. Finally, we validate the robustness of \sys on different hardware types, degree of changes, safe starting points. 



\noindent\textbf{Baselines}: The baselines are presented below:
\begin{itemize}[leftmargin=*]
\item Default: The default knobs configuration provided by experienced DBA, which is expected to be robust across workloads.
\item \sys: \sys is our safe and contextual tuner. We implement \sys's prediction model with GPy library.

\item Bayesian Optimization (BO): BO is black-box optimization approaches, widely used in database knobs tuning ~\cite{DBLP:journals/pvldb/DuanTB09, DBLP:conf/sigmod/AkenPGZ17, DBLP:conf/hotstorage/KanellisAV20,DBLP:journals/pvldb/AkenYBFZBP21,DBLP:conf/sigmod/ZhangWCJT0Z021}. We use similar design with OtterTune~\cite{DBLP:journals/pvldb/DuanTB09}: Gaussian process as its prediction model and UCB as its acquisition functions. It's also implemented with GPy library.
\item Deep Deterministic Policy Gradient (DDPG): DDPG is a policy-based model-free reinforcement learning agent which is used to tune the database knobs configuration ~\cite{DBLP:conf/sigmod/ZhangLZLXCXWCLR19, DBLP:journals/pvldb/LiZLG19}. The DDPG algorithm is implemented using PyTorch library with its neural network architecture borrowed from CDBTune~\cite{DBLP:conf/sigmod/ZhangLZLXCXWCLR19}.
\end{itemize}


\noindent\textbf{Workload}:
We choose three workloads with different characteristics from well-known database benchmarks and one real-world workload. The three workloads are TPC-C, Twitter from OLTP-Bench~\cite{DBLP:journals/pvldb/DifallahPCC13} and OLAP workload JOB~\cite{DBLP:journals/pvldb/LeisGMBK015}. TPC-C is a traditional OLTP benchmark characterized by write-heavy transactions with complex relations. 
It is the current industry standard for evaluating the performance of the OLTP system \cite{DBLP:books/mk/gray93/Raab93}.  Twitter is extracted from web-based applications, characterized by heavily skewed many-to-many relationships and non-uniform access. JOB is an analytical workload with 113 multi-join queries, characterized by realistic and complex joins. In order to fully evaluate the benefits of tuning, we use unlimited arrival rate for Twitter and TPC-C, as ~\cite{DBLP:journals/pvldb/DuanTB09, DBLP:conf/sigmod/AkenPGZ17, DBLP:conf/hotstorage/KanellisAV20,DBLP:conf/sigmod/ZhangLZLXCXWCLR19, DBLP:journals/pvldb/LiZLG19} did. In \textit{static workload} setting, we fix the queries composition. For TPC-C and Twitter, the transaction weight is set to the default value. For JOB, we execute ten fixed queries from the query set every tuning iteration. In \textit{dynamic workload} setting, we construct changing queries composition along with the time interval.  In \textit{transactional-analytical} setting, we alternate the execution of TPC-C and JOB workload every 50 time intervals with their queries composition changing.  In \textit{real-workload workload} setting, the queries composition and arrival rate are constantly changing.

\noindent\textbf{Setup}:
We use version 5.7 of MySQL RDS. We tune 40 dynamic knobs whose modification do not need the restart of MYSQL, as the restart is not acceptable in the online business application. The 40 knobs are chosen according to their importance by DBA. The experiments run on cloud instances with 8 vCPU and 16GB RAM. We also use a smaller instance (4 vCPU and 8GB RAM) and a larger instance (16 vCPU and 32GB RAM) to validate the robustness of \sys. Experiments are run on the 8vCPU instance unless otherwise mentioned. We use the DBA default configuration s the initial safety set and its 
performance as safety threshold.  For fairness, the initial safety set is also added as the training data to the other baselines. As the DBA default is a relatively good start points for \sys, we also evaluate \sys's performance using MYSQL default configuration as initial safety set and its performance as safety threshold. 
For workload featurization in \sys, we use a one layer bidirectional LSTM as encoder and the dimension of query embedding is set to six. The weights of the encoder and decoder are shared. We use queries from 10 workloads in OLTP-Bench, JOB and our real-world workload trace to train the auto-encoder.  The training data has $\sim$ 40 thousand quires, 403 distinct templates. It's noted that the training set of the encoder can be enlarged to enhance the generality, .e.g, \cite{DBLP:conf/sigmod/ZolaktafMP20} uses Sloan Digital Sky Survey (SDSS) query workload which contains $\sim$ 618 thousand queries. With the six dimension query embedding, query arrival rate, three dimension query optimizer statists, we obtain a ten dimension context representation.


 
\noindent\textbf{Evaluating Metrics}: 
 We evaluate the tuning methods from the perspective of safety and the performance gain of using knobs tuning.  
 For safety, we count the number of unsafe knobs recommendations (\#unsafe) and the number of system failures (\#failures) within the tuning period. As discussed, we use the database performance under default configuration as the safety threshold. The unsafe knobs are knobs whose performance is lower than the default performance.
 For the  performance gain, we calculate the cumulative performance improvement obtained through tuning ~\cite{DBLP:conf/kdd/FekryCPRH20}. The improvement is calculated by comparing the performance after tuning with the the default configuration performance. For OLTP workload, the improvement is measured by the increase in the number of transactions processed by the database. For OLAP workload, the improvement is measured by the savings in execution time. For \textit{static workload} setting, we can also evaluate the search time required to get close to the estimated optimal configuration and the maximum improvement.
 
 
   \begin{figure}[t]
\centering
    \includegraphics{plot/dynamic_workload/time.pdf}
\caption{Inference time of different tuning approaches}
\label{fig:time}
\vspace{-0.255cm}
\end{figure} 

\begin{table*}
\footnotesize
\setlength\tabcolsep{2pt}
\caption{Statists when tuning static workload: For each workload, bold face indicates the best value. Search Step in  is the iteration needed until finding a configuration within $10\%$ of the estimated optimum, $\backslash$ means such configuration is not found. }\label{tab:fix}
\begin{tabular}{@{}cccccccccccccccc@{}}
\toprule
                             & \multicolumn{5}{c}{\textbf{\sys}}                                                           & \multicolumn{5}{c}{\textbf{BO}}                                                       & \multicolumn{5}{c}{\textbf{DDPG}}                           \\
\textbf{Workload}            & \#Unsafe   & \#Fail     & Avg Improv.      & Max Improv.      & Search Step                       & \#Unsafe & \#Fail & Avg Improv. & Max Improv.      & Search Step                      & \#Unsafe & \#Fail & Avg Improv. & Max Improv. & Search Step \\ \midrule
\multicolumn{1}{c|}{TPC-C}   & \textbf{0} & \textbf{0} & \textbf{8.15\%}  & 17.03\%          & \multicolumn{1}{c|}{176}          & 103      & 2      & -10.95\%    & \textbf{19.99\%} & \multicolumn{1}{c|}{\textbf{74}} & 136      & 2      & -15.28\%    & 16.66\%     & 76          \\
\multicolumn{1}{c|}{Twitter} & \textbf{2} & \textbf{0} & \textbf{16.69\%} & \textbf{48.18\%} & \multicolumn{1}{c|}{\textbf{129}} & 70       & 15     & -9.51\%     & 43.43\%          & \multicolumn{1}{c|}{158}         & 197      & 3      & -78.76\%    & 35.79\%     & $\backslash$          \\
\multicolumn{1}{c|}{JOB}     & \textbf{1} & \textbf{0} & \textbf{4.90\%}  & \textbf{11.67\%} & \multicolumn{1}{c|}{\textbf{141}}            & 195      & 6      & -929.89\%    & 7.77\%          & \multicolumn{1}{c|}{$\backslash$}  & 197      & 8      & -1191.18\%   & 7.60\%     & $\backslash$          \\ \bottomrule
\end{tabular}

\end{table*}
 
 




  \begin{figure*}
\centering
    \includegraphics{plot/fix_workload/performance_all.pdf}
\caption{Performance when tuning static workload: minimal throughput (0) and maximal latency (200) denote system failure }
\label{fig:fix-performance}
\end{figure*}
\vspace{0.03cm}

 \begin{figure}[htbp]
\centering
    \includegraphics{plot/fix_workload/imporve_all.pdf}
\caption{Cumulative improvement for static workload}
\label{fig:fix-improvement}
\end{figure}


\subsection{Algorithm Overhead}

 As the auto-tuners are deployed in the backend tuning cluster, most of their computation resource expenditure will not affect online database's performance. But long inference time of models will obstruct their responds to changing workload.
 For BO and DDPG, the inference time is consist of: (1) statistics collection, (2) model fitting, and (3) model probe. For \sys, the time also includes featurization. Figure \ref{fig:time} shows the inference time along iterations when tuning Workload JOB. The inference time for BO increases exponentially with the tuning iteration, as Gaussian process suffers from cubic complexity to  the sample size.  Instead, \sys only uses the data samples in the predicted context subspace to fit prediction model , therefore its inference time is bounded as discussed in Section \ref{sec:context-partition}.  %The time of featurization in \sys is about 57.7 ms and the time of periodic context space partition is about 3.2ms $\sim$ 33.8ms. 
  

 
 \subsection{Evaluation on Static Workload}
 We first evaluate \sys when tuning static workload against 3 approaches (DBA default, BO, DDPG). 
 Tuning static workload is a typical scenario where existing approaches function well to search the optimal configurations. The aim of this experiment is to assess the search efficiency of \sys with safety guarantee.  
 
 \noindent\textbf{\sys reduces the unsafe recommendation significantly with search time comparable to the state of the art tuning systems.}
  Figure \ref{fig:fix-performance} plots the performance of different tuning approaches and Table \ref{tab:fix} shows their statistics where DBA default is used as a baseline to calculated the improvement. 
  BO and RL are designed to search for the global optimum without any safety constraints. In the aspect of efficiency, \sys's performance is comparable to BO, while better than RL in all cases. Although, \sys's safety consideration makes the exploration slower, the restricting of space search localizes good solutions and improves convergence in Twitter's and JOB's cases. As shown in the statistics, \sys is very unlikely to apply unsafe configurations, while, as expected, BO and RL violates the safety constraint considerably. 
 
 % Given the large configuration space, existing auto-tuners always have a chance to explore the configuration worse than the default.
 \noindent\textbf{\sys is always cost-effective.}
 Figure \ref{fig:fix-improvement} shows the cumulative improvement  when applying the configurations determined iteratively by the tuning algorithms to the online database. We also use the DBA default as a baseline to calculate the improvement. The cumulative improvement indicate the benefit of knobs tuning from the online's perspective. Surprising, within the 200 iterations, applying BO and DDPG to tune the online system causes the total performance downgrade (negative improvement), compared to using DBA default directly. The reason behind is that BO and RL have a large cost of exploring the search space for a good configuration. If the workload only recurs  several times (i.g, within 200 iterations in this cases), their tuning cost can not be amortized.  What's more, given the large configuration space, they always have a chance to explore the configuration worse than the default, making the amortization more difficult. As \sys is designed to ensure safety (better than default) throughout the whole tuning process, the benefit of adapting \sys is guaranteed.
  
 
 
\begin{figure}[t]
\centering
    \includegraphics{plot/dynamic_workload/mix.pdf}
\caption{Transaction weight}
\label{fig:dynamic-weight}

\end{figure}


 \begin{figure}[htbp]
\centering
    \includegraphics{plot/dynamic_workload/imporve_all.pdf}
\caption{Cumulative improvement and safety statistics when tuning dynamic workload}
\label{fig:dynamic-improvement}
\vspace{0.01cm}
\end{figure}

  
\begin{figure*}
\centering
    \includegraphics{plot/real/performance_all.pdf}
\caption{Performance when tuning OLTP-OLAP cycle and real-world workload}
\label{fig:real-performance}

\end{figure*}
  
  
  
    \begin{figure}[t]
\centering
    \includegraphics{plot/real/imporve_all.pdf}
\caption{Cumulative improvement and safety statistics when tuning  workload with OLTP-OLAP circle}
\label{fig:real-improvment}

\end{figure}


  
     \begin{figure}[htbp]
\centering
    \includegraphics{plot/real/imporve_all.pdf}
\caption{Cumulative improvement and safety statistics when tuning real-world workload}
\label{fig:real-improvment2}

\end{figure}

 
 
  \subsection{End-to-end Evaluation}
 In this section, we evaluate \sys tuning evolving workloads. In order to mimic all the possible changes, we construct \textit{dynamic workloads} setting with query distribution changing and \textit{transactional-analytical} setting  with query type changing. We also test \sys in production environment in \textit{real-workload workload} setting with the changes of query arrival rate and distribution. For TPC-C workload and  real-workload workload, the data size and distribution  is changing constantly during the tuning process due to the DML of workload.
  We seek to address the following questions: Can \sys find workload-specific configuration better than DBA default? Can \sys adapt to all kind of changing workloads, while reliably respecting the safety requirement? How does it compare against existing tuning approaches?
   
 
 \subsubsection{Evaluation on Dynamic Workload}\label{sec:exp-dynamic}
 
 we construct changing queries composition along with the tuning interval.
For TPC-C and Twitter, we change the transaction weights every interval, using OLTP-Bench. To simulate the gradual change, the  transaction weights is sampled from a normal distribution with a sine function of time as mean and a standard deviation of $10\%$, as shown in figure \ref{fig:dynamic-weight} (a). For TPC-C, the four transactions are NewOrder, Payment, OrderStatus, Delivery, respectively. For Twitter, they are GetTweet, GetTweetsFromFollowing, GetFollowers, GetUserTweets, respectively. For JOB, we execute ten queries, five out of which are resampled every time interval from the query set. As TPC-C is a write-heavy workload, its underlying data is also changing (.e.g, its data size is $\sim$ 18 GB at the beginning of tuning, and $\sim$ 28 GB after 400 tuning iterations). And the transactions of Twitter and JOB are read-only, therefore their underlying data is not changed. We also conduct experiments with more drastic changes of workload (Figure \ref{fig:dynamic-weight} (b)) and more hardware types to evaluate the robustness of \sys in Section \ref{sec:analysis}.

\noindent\textbf{\sys finds workload-specific configuration better than reasonably  hand-tuned configuration.} As shown in Figure \ref{fig:dynamic-improvement}, applying \sys leads to $11.61\% \sim 23.24\%$ improvement on average, compared to the DBA default. And \sys's cumulative performance gain is much larger than existing approach (BO and DDPG). BO uses observations, $\{\theta_i, y_i\}_1^{t}$ to fit its prediction model, ignoring the changing environment factors that  also affects the database performance. When workload changes, BO struggles to learn the good configuration. DDPG can fin-tune its model when the environment changes, but fin-tuning a neural network needs lots of samples and the adaption can not hold pace with the changing environment.

\noindent\textbf{ \sys reliably respects the safety requirement when tuning online system.} Restricting the optimization space in a safety set is not a trivial task for online tuning system, since the changes of workloads may cause the shifting of safety set. 
Right part of Figure \ref{fig:dynamic-bar} shows the count of unsafe configurations and system failures when tuning the online system of different approaches.  None of system failures  arises when applying \sys, while BO and DDPG cause several system failures, which is unacceptable for the production environment.  BO and DDPG have $27\% \sim 81\%$ unsafe knobs recommendations within the 400 tuning intervals. \sys controls the unsafe knobs ratio lower than $2\%$ and the performance of unsafe knobs is within $10\%$ deviation from the safety threshold. This is contributed to the black-and-white safety assessment and the subspace expanding strategy of \sys, which we will analyze in details with ablation study (Section \ref{sec:ablation-safe}).

  



  
 % Please add the following required packages to your document preamble:
% \usepackage{booktabs}

 \subsubsection{Evaluation on Transactional-Analytical Cycle}
 We simulate a daily transactional-analytical workload cycle by alternating the execution of TPC-C and JOB workloads. And the transaction weight of TPC-C and query composition of JOB are changed every time interval, like in Section \ref{sec:exp-dynamic}. We use 99\% latency as optimization objective. The workload characterization of TPC-C (OLTP, write-heavy) and JOB (OLAP, complex joins) are significantly different and the evolve between the two workload is violent, tuning such a online system with safety guarantee is challenging.
 Figure \ref{fig:real-performance} (a) shows the performance of \sys and DBA default configuration. The workload starts as TPC-C and switches to JOB after 100 tuning iterations repeatedly.  
 As interaction with the online database system,  \sys begins to finds configurations with larger improvement than the DBA default gradually as shown in the zoom-in plot. When switching to JOB, \sys takes some iterations to exploration in the configuration space, meanwhile several unsafe knobs recommendations slightly larger than the safety threshold occur. Then, \sys finds good configuration adaptively (.e.g, larger sort buffer size,  treating NULL values unequally  when collecting statistics to encourage to use index)
 After 300 tuning iterations, when switching from TPC-C to JOB workload again, \sys selects the prediction model fit with data in the context subspace for JOB and recommend good knobs configurations more quickly. Figure \ref{fig:real-improvment} shows the accumulative improvement and safety statists of the different approaches (\sys, BO and DDPG). Similarly with previous evaluation, adopting \sys leads to performance improvement with safety guarantee, while other approaches fail.     

 
 \subsubsection{Evaluation on Production Workload}
 
 
\begin{figure}[t]
\centering
    \includegraphics{plot/ablation/context_imporve_all}
\caption{Ablation study  on context space design}
\label{fig:ablation-contex-improvement}

\end{figure}

  \begin{figure}[t]
\centering
    \includegraphics{plot/ablation/safe_imporve_all}
\caption{Ablation study  on safe exploration}
\label{fig:ablation-safe-improvement}

\end{figure}
 
 
 \subsection{Analysis of \sys}\label{sec:analysis}
 In order to safely explore good configurations in dynamic environment, we carefully design \sys with learned context space and safe exploration strategy. We now evaluate the two parts of design in \sys.
  
 \subsubsection{Ablation study  on Context Space Design}
We remove certain components of context space design (featurization of workload and data changes, context space partition) in \sys to understand the contribution of those components to the overall system.  We compare (1) \sys, (2) \sys-w/o-workload, removing workload embedding from context feature, (3) \sys-w/o-data, removing optimizer statistics (data change) from context feature, (4) \sys-w/o-partition, removing context space partition.
The experiments are conducted in dynamic TPC-C and JOB with the same construction as in Section \ref{sec:exp-dynamic}. Figure \ref{fig:ablation-contex-improvement} shows the cumulative improvement and safety statistic of those baselines.  For the read-only workload JOB where no data changes occurs, \sys-w/o-data exceeds \sys slightly because its context dimension decreases with no information loss, meaning that generalizing over the context dimension is easier. However, when data change occurs as in TPC-C workload, \sys beats the other baselines, as the combination of workload and data changes give a comprehensive abstraction of the dynamics of environment. \sys-w/o-partition is  inferior to \sys in TPC-C and JOB. As \sys can chooses similar context space and prevent the "negative transfer" from distant contexts. 


  \begin{figure*}
\centering
    \includegraphics{plot/dynamic_workload/performance_twitter.pdf}
\caption{Tuning Twitter workloads with difference degree of changes}
\label{fig:dynamic-twitter}

\end{figure*}


  \begin{figure}[t]
\centering
    \includegraphics{plot/dynamic_workload/instances.pdf}
\caption{Tuning TPC-C workload on different type of instances}
\label{fig:dynamic-instance}

\end{figure}

  \begin{figure}[t]
\centering
    \includegraphics{plot/dynamic_workload/performance_mysql.pdf}
\caption{Starting from Mysql Default}
\label{fig:vary-start}

\end{figure}



 \subsubsection{Ablation Study on Safe Exploration}\label{sec:ablation-safe}
 To safely tune the database in dynamic environment, \sys 
 uses Gaussian predictions (black-box knowledge), accompanying domain knowledge (white-box knowledge) to assess the safety of configuration and gradually expands the optimization subspace. To analyze their functionality, we compare: (1) \sys, (2) \sys-w/o-white, removing black-box safety assessment (3) \sys-w/o-black, removing white-box safety assessment, (4)\sys-w/o-subplace, optimizing in the whole configuration space, (5) \sys-w/o-safe, removing all the safety strategy, i.e., contextual Bayesian Optimization in Section \ref{sec:context-model}. As shown in Figure \ref{fig:ablation-safe-improvement}, \sys precedes the other baselines in both improvement and safety guarantee. We can make the following observations: 
  (1) The black-box knowledge largely reduces the unsafe knobs recommendations. \sys-w/o-black's unsafe recommendations is much more than \sys-w/o-white. This is because the limited domain rules only covers a small subset of unsafe cases and fails to capture the complex and high-dimension relationship between configuration, environment and system performances. 
 (2) The white-box knowledge assists to filter the unsafe configurations.  We find that the unsafe recommendation in \sys-w/o-white is mainly cased by the knobs without intrinsic ordering, e.g., thread\_concurrency. Thread\_concurrency defines the maximum number of threads permitted inside of InnoDB. But a value of 0 (the BDA default value) is interpreted as infinite concurrency (no limit).  The Gaussian process prediction model depends on the natural ordering property and smoothies of space. When \sys-w/o-white expands the safe space, it is very likely to try a value near zero, like one, casing the database performance to drop due to the lack of computing resources. \sys has domain rules to filter the value of thread concurrency less than half of the number of virtual CPUs, preventing the unsafe case. (3) Optimizing in promising sub-space instead of the whole configuration space can enhance the safety and localize good configurations.  The number of unsafe recommendation in \sys-w/o-subplace is larger than in \sys. As we discussed, it's hard to evaluate the safety of configuration in the whole space, instead, the prediction of contextual Gaussian process is trusted in a small trust region. Besides, the performance gain of \sys-w/o-subplace is much lower than baselines optimizing in subspaces. This is because the global optimization approach (.i.e., \sys-w/o-subplace) over-explores the boundary of configuration space, especially in the high dimensional ~\cite{DBLP:conf/nips/WangFT20}. (4) Without all the safety consider, \sys-w/o-safe has the worst performance and its tuning cost can not be amortized.

  
 \subsubsection{Varying Degree of Changes}
  \sys recommends configuration based on the context of environment. In reality, the change of workload and the underlying data is a gradual process and \sys generalizes over the similar contexts.  When degree of changes increase, safely tune the online database becomes more challenging. We evaluate the performance of \sys tuning Twitter under difference degree of changes. Figure \ref{fig:dynamic-twitter} (a) shows the performance with workload of transaction weight sampled with $10\%$ variance and Figure \ref{fig:dynamic-twitter} (b)  shows workload with $30\%$ variance (more drastic changes).  The line of DBA default's performance is more fluctuating in Figure \ref{fig:dynamic-twitter} (b) as expected.
  In summary, \sys achieves $23.24\%$ improvement compared to DBA default with 2 unsafe configurations when tuning workload with $10\%$ variance and $18.74\%$ improvement with 5 unsafe configurations when tuning workload with $30\%$, showing the robustness of \sys for workload changes.

 \subsubsection{Varying Hardware Types}
 To validate the robustness of \sys on different hardware types, we apply \sys to tune dynamic Twitter on three different hardware instances: (1) Small, an instance with 4 vCPU and 8GB RAM, (2) Medium: an instance with 8 vCPU and 16GB RAM, (3) Large, 16 vCPU and 32GB RAM. Figure \ref{fig:dynamic-instance} shows the cumulative improvement and statistics of unsafe knobs recommendation. The count of system failures is omitted, since none failure occurs during tuning. Basically, \sys safely tunes the databases and achieves performance gain.  On the small instance, the number of unsafe recommendation is a bit larger, because limited machine capacity causes the more difficult safety requirement.  
  Meanwhile, as the instance's capacity grows, the unsafe knobs count decreases and cumulative improvement grows.
  

\subsubsection{Varying Initial Safety Set and Safety Threshold}
 During online tuning, \sys begins the exploration of configuration space from the initial safety set.
 In the above part of evaluation, we use the DBA default as the initial safety set and its performance as safety threshold. This is because online tuning is meaningful in production environment, only when the tuning can leads to performance gain compared to a relative robust configuration (.i.e., the DBA default). Otherwise, it's more beneficial to simply fix the knobs configuration to the DBA default. And the above evaluation shows the performance gain of adopting \sys compared to the the DBA default. However, one question remains, that is, can \sys recommend good configurations with bad starting point? In this part, we use Mysql default configuration as the initial safety set and its performance as the safety threshold. As shown in Figure \ref{fig:vary-start}, the performance of the Mysql default configuration is inferior to the  DBA default. One of the main difference between the Mysql Default and the DBA default is that the Mysql default sets the buffer pool size  128 MB while DBA default sets the buffer pool size about 13 GB.
 When starting at the Mysql default, \sys successfully finds configuration better than the Mysql default and gradually it achieves superior performance than the DBA default, showing the ability of \sys to tune the online system adaptively with changing workload. And given bad starting configuration, \sys can still find good close-to-optimal configurations.
 
 \input{case_study}

 


==> intro_old.tex <==
\section{Introduction}
\begin{figure}
\centering
    \includegraphics{plot/intro/motivation.pdf}
\caption{Motivating Examples}
\label{fig:motivation}
\end{figure}

Modern database management systems (DBMS) have dozens of configurable knobs that control its runtime behaviors ~\cite{DBLP:journals/pvldb/DuanTB09}.  Knobs settings for the workload of an application affects the performance of DBMSs (e.g., higher throughput and lower latency). Finding the optimal knobs configuration for a given workload is an NP-hard problem ~\cite{DBLP:conf/sigmetrics/SullivanSP04}. Given this, database administrators (DBAs) put considerable effort into tuning these knobs based on experience. 
 
 
 In the cloud environment, various workloads and users schemas make tuning more challenging.  Each workload has particular characteristics in terms of access distribution and resource usage. Therefore, there is no global optimal configuration, instead a workload-specific optimal configuration ~\cite{DBLP:conf/sigmod/IdreosK19, DBLP:conf/kdd/FekryCPRH20}. Further exacerbating this problem is that the workloads for real-world applications are never static \cite{DBLP:conf/sigmod/MaAHMPG18}. Figure \ref{} shows the workload pattern of a real-world database application trace. Furthermore, the underlying data size and distribution are also constantly changing due to the frequent data modification language statements (DML). Such changes can lead to significant changes in the workload’s behavior under particular configurations.


Recently, some studies on automatic knobs configuration use machine learning techniques designed for optimizing a given workload. During training, the tuner outputs knobs configuration according to a specific model or policy. Then, the configuration is applied to the database, and workload replay is triggered. After the replay is finished, the database performances metrics are collected to update the model. The tuner learns the exemplary configuration by exploring the configuration space. Such a training process typically repeats hundreds to thousands of iterations.  Once trained, it is assumed that the tuner can predict close-to-optimum configurations for the given workload.

However, the above approach has two severe limitations. 
 First, the prediction of the automatic tuner is only effective as long as workloads and their runtime environment during prediction never drift too far from conditions during training. As discussed above, a significant number of real-world situations do not fit this assumption. The composition and volume of the queries in an application’s workload change over time. The predication may soon become inappropriate. 
Second, during training, it is inevitable for the tuner to apply the bad knobs configuration to the database, causing the system performance downgrade. Figure \ref{fig:motivation} (a) shows the existing automatic knobs tuning approach (OtterTune and CDBTune) tuning the workload TPCC in MYSQL. OtterTune utilizes Bayesian Optimization to learn suitable configurations by exploration and exploitation, and CDBTune adopts reinforcement learning to learn the tuning policy by trials-and-error. Although configurations better than the default are found, 50\%\textasciitilde70\% of configurations recommended by the tuner are worse than the default performance. The tuning even causes 2 system failures by configuring more memory than the database can allocate or setting a too small threshold(like the maximum rows a statement can examine), making the transactions unable to be processed. For the existing approaches explore the bad configurations is part of learning. However, such bad exploration exposes enormous risks to the database end-users, and the performance downgrade is not acceptable for the mission-critical application. Therefore, the existing automatic tuner is mainly deployed offline on a second copy of the database to tune benchmark workloads or sample workload from the real-world application. Such offline tuning can not respond to the constantly changing workload online. Moreover, users who conduct offline tuning have to buy a copy instance, largely increasing the Total Cost of Ownership for using cloud databases.
%(TODO): highlight offline tuning cost

Those limitations cause the existing automatic tuning in the cloud risky and expensive. 
 From this perspective, a practical automatic tuner can be deployed online faced with the constantly changed conditions in the production without exposes vast risks to the end-users. The tuner has to fulfill two requirements:
 
 \noindent\textbf{Dynamic}: Instead of assuming a given workload, the automatic tuner should be capable of responding to the constantly changing workload and underlying data in the cloud. 
 
  \noindent\textbf{Safe}: To be deployed online, the tuner should recommend knobs without downgrading the system performance during the whole optimization process.  
  
Therefore, the online tuning can be formulated as a contextual bandit problem with safety constraints for every tuning iteration.
 To address this problem, we propose an online tuning system, \sys, which can tune the databases safely in the constantly changing cloud environment. OnlineTune is based on contextual Bayesian optimization (BO)~\cite{DBLP:conf/nips/KrauseO11}.  The main idea of Contextual BO is to learn how the changes in both input and context affect the system’s output and use the learned relationships to find the optimum input for each varying context. Using contextual BO, OnlineTune optimizes the database adaptively to varying workloads. However, the BO algorithm suffers from the curse of dimensionality in the high-dimensional search space, and its success is limited to a few thousand evaluations data \cite{Wang2018BatchedLB} and less than 15 parameters \cite{DBLP:conf/icml/NayebiMP19}. Directly deploying the conventional contextual BO algorithm can not achieve satisfactory predictions in the online tuning scenario due to increasing tuning evaluations data in the cloud and the high-dimension knobs configuration space of databases. Moreover, it also over-explores the bad configuration space as the existing automatic tuner does.
This has motivated us to scale up contextual BO by carefully breaking down its optimization space. For the context space, a space partition is learned, and for every incoming context, only the evaluation data in its predicted partition is selected as training data. For configuration space, we convert the high-dimension optimization to a sequence of iteratively solving low-dimensional subspace problems that can be modeled efficiently. 
 
 Furthermore, to avoid the recommendation of bad knobs, a safe exploration strategy is proposed by combining the black-box and white-box knowledge. As the low-dimension subspace can be efficiently discretized, OnlineTune maintains a safe candidate set for each subspace. OnlineTune uses the lower bound of the confidence interval from Gaussian precess (black-box knowledge) in the subspace to filter the unsafe knobs configurations.  It safely explores the subspace, starting from configurations similar to those known to be safe. Proceeding this way, the safe subspace is expanded, facilitating further exploration. Besides, the white-box knowledge in the database domain can serve as a guide to filter the unsafe configurations, e.g., the knobs configurations exceed the physical capacity of any of the machine’s resources.  This white-box knowledge is a rule-based heuristic, which can be experience from DBA or existing tuning tools for database systems ~\cite{MySQLTuner, pgtune, DBLP:conf/cidr/DiasRSVW05}. A relaxing strategy is proposed to reduce the rule against black-box knowledge to a certain degree to prevent the ineffective rule from impeding optimization.
 
 
 
 
Specifically, we make the following contributions:
 \begin{itemize}
 \item To deal with the challenges in real DBMS scenarios with constantly changing workload, we define the online knobs tuning problem and formulate it as a contextual bandit problem with safety constraints for every tuning iteration.
 
 \item We propose a context featurization model that featurizes the workloads and underlying data to a vector. Contextual Bayesian optimization is adopted to optimize against constantly changing context. To scale up contextual BO with increasing evaluation data in the cloud and high-dimension knobs configuration space of the database, we propose to break down both the context and configuration spaces into subspaces by space partition and local modeling.
 
 \item We propose a safe exploration strategy by combining the black-box and white-box knowledge, largely reducing the recommendation of bad configurations when using automatic tuning. 

 \item We implement the proposed method and evaluate on standard benchmarks and real workloads. Compared with the state-of-the-art, ....
 \end{itemize}
 
  



   
  

